Economic Valuation and Pricing of Inertia in Inverter-Dominated Power Systems

This paper studies the procurement and pricing of inertial response using a frequency-constrained unit commitment formulation, which co-optimizes the provision of energy and inertia services while accounting for their complementary properties. The proposed approach builds on a two-step process that allows to differentiate between the units being online for energy purposes and the ones committed additionally solely for inertia provision. Subsequently, three novel pricing and payment schemes that reimburse inertia providers in a transparent and fair manner according to their individual participation are proposed. The analysis considers both synchronous and converter-based generators and provides insights regarding the impact of each pricing scheme on total system cost, as well as on the investment signals for technologies capable of offering affordable inertial response. The results show that all three methods will have a beneficial impact on frequency stability and aid the operator in ensuring system reliability, whereas the policy implications to different inertia providing units will vary between the payment schemes.

==> Economic Valuation and Pricing of Inertia in Inverter-Dominated Power Systems - Journal Paper (Matthieu)/tables/table1.tex <==
\huge
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c}
    \thickhline
    \cellcolor{black!10}$\Huge\boldsymbol{H\text{\textbackslash}G}$& $\Huge\boldsymbol{G_1}$ & $\Huge\boldsymbol{G_2}$ & $\Huge\boldsymbol{G_3}$ & $\Huge\boldsymbol{G_4}$ & $\Huge\boldsymbol{G_5}$ & $\Huge\boldsymbol{G_6}$ & $\Huge\boldsymbol{G_7}$ & $\Huge\boldsymbol{G_8}$ & $\Huge\boldsymbol{G_9}$ & $\Huge\boldsymbol{G_{10}}$ & $\Huge\boldsymbol{G_{11}}$ & $\Huge\boldsymbol{G_{12}}$ & $\Huge\boldsymbol{G_{13}}$ & $\Huge\boldsymbol{G_{14}}$ & $\Huge\boldsymbol{G_{15}}$ & $\Huge\boldsymbol{G_{16}}$ & $\Huge\boldsymbol{G_{17}}$ & $\Huge\boldsymbol{G_{18}}$ & $\Huge\boldsymbol{G_{19}}$ & $\Huge\boldsymbol{G_{20}}$ \\
    \thickhline
$\Huge\boldsymbol{H_1}$ & 	\cellcolor{myGreen!25}915 & 	\cellcolor{myGreen!25}915 & 	\cellcolor{myGreen!25}926 & 	\cellcolor{myGreen!25}1164 & 	\cellcolor{myGreen!25}891 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}1531 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}915 & 	\cellcolor{myGreen!25}915 & 	\cellcolor{myGreen!25}926 & 	\cellcolor{myGreen!25}1164 & 	\cellcolor{myGreen!25}891 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}1531 & 	\cellcolor{myGreen!25}959	\\ \thickhline
$\Huge\boldsymbol{H_2}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_3}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_4}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_5}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_6}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_7}$ & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{red!25}-161 & 	\cellcolor{myGreen!25}116 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}69 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-46 & 	\cellcolor{red!25}-96 & 	\cellcolor{myGreen!25}116 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}69 & 	\cellcolor{myGreen!25}171	\\ \thickhline
$\Huge\boldsymbol{H_8}$ & 	\cellcolor{red!25}-143 & 	\cellcolor{red!25}-143 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}274 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{myGreen!25}145	\\ \thickhline
$\Huge\boldsymbol{H_9}$ & 	\cellcolor{red!25}-143 & 	\cellcolor{red!25}-143 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{myGreen!25}145	\\ \thickhline
$\Huge\boldsymbol{H_{10}}$ & 	\cellcolor{red!25}-143 & 	\cellcolor{red!25}-143 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{myGreen!25}145	\\ \thickhline
$\Huge\boldsymbol{H_{11}}$ & 	\cellcolor{myGreen!25}65 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{myGreen!25}65 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}94 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}39 & 	\cellcolor{myGreen!25}145	\\ \thickhline
$\Huge\boldsymbol{H_{12}}$ & 	\cellcolor{myGreen!25}70 & 	\cellcolor{myGreen!25}70 & 	\cellcolor{red!25}-23 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}105 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}54 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}70 & 	\cellcolor{myGreen!25}70 & 	\cellcolor{myGreen!25}217 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}105 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}54 & 	\cellcolor{myGreen!25}158	\\ \thickhline
$\Huge\boldsymbol{H_{13}}$ & 	\cellcolor{myGreen!25}70 & 	\cellcolor{myGreen!25}70 & 	\cellcolor{red!25}-23 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}105 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}54 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}70 & 	\cellcolor{myGreen!25}70 & 	\cellcolor{myGreen!25}217 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}105 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}54 & 	\cellcolor{myGreen!25}158	\\ \thickhline
$\Huge\boldsymbol{H_{14}}$ & 	\cellcolor{myGreen!25}166 & 	\cellcolor{myGreen!25}166 & 	\cellcolor{red!25}-442 & 	\cellcolor{red!25}-1091 & 	\cellcolor{myGreen!25}313 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}325 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}166 & 	\cellcolor{myGreen!25}166 & 	\cellcolor{myGreen!25}167 & 	\cellcolor{red!25}-1091 & 	\cellcolor{myGreen!25}313 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}325 & 	\cellcolor{myGreen!25}401	\\ \thickhline
$\Huge\boldsymbol{H_{15}}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{red!25}-442 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_{16}}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{red!25}-442 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_{17}}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{red!25}-442 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_{18}}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_{19}}$ & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}73 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}211 & 	\cellcolor{myGreen!25}214 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}346 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}394 & 	\cellcolor{myGreen!25}504	\\ \thickhline
$\Huge\boldsymbol{H_{20}}$ & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}378 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}1107	\\ \thickhline
$\Huge\boldsymbol{H_{21}}$ & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}378 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}1107	\\ \thickhline
$\Huge\boldsymbol{H_{22}}$ & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}378 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}1107	\\ \thickhline
$\Huge\boldsymbol{H_{23}}$ & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}378 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}1107	\\ \thickhline
$\Huge\boldsymbol{H_{24}}$ & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}378 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}464 & 	\cellcolor{myGreen!25}377 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}631 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}872 & 	\cellcolor{myGreen!25}1107	\\
    \arrayrulecolor{black}\thickhline
\end{tabular}
 }

==> Economic Valuation and Pricing of Inertia in Inverter-Dominated Power Systems - Journal Paper (Matthieu)/tables/table2.tex <==
\huge
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c}
    \thickhline
    \cellcolor{black!10}$\Huge\boldsymbol{H\text{\textbackslash}G}$& $\Huge\boldsymbol{G_1}$ & $\Huge\boldsymbol{G_2}$ & $\Huge\boldsymbol{G_3}$ & $\Huge\boldsymbol{G_4}$ & $\Huge\boldsymbol{G_5}$ & $\Huge\boldsymbol{G_6}$ & $\Huge\boldsymbol{G_7}$ & $\Huge\boldsymbol{G_8}$ & $\Huge\boldsymbol{G_9}$ & $\Huge\boldsymbol{G_{10}}$ & $\Huge\boldsymbol{G_{11}}$ & $\Huge\boldsymbol{G_{12}}$ & $\Huge\boldsymbol{G_{13}}$ & $\Huge\boldsymbol{G_{14}}$ & $\Huge\boldsymbol{G_{15}}$ & $\Huge\boldsymbol{G_{16}}$ & $\Huge\boldsymbol{G_{17}}$ & $\Huge\boldsymbol{G_{18}}$ & $\Huge\boldsymbol{G_{19}}$ & $\Huge\boldsymbol{G_{20}}$ \\
    \thickhline
$\Huge\boldsymbol{H_1}$ & 	\cellcolor{myGreen!25}168 & 	\cellcolor{myGreen!25}168 & 	\cellcolor{myGreen!25}134 & 	\cellcolor{red!25}-153 & 	\cellcolor{myGreen!25}324 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}364 & 	\cellcolor{red!25}-1222 & 	\cellcolor{myGreen!25}168 & 	\cellcolor{myGreen!25}168 & 	\cellcolor{myGreen!25}134 & 	\cellcolor{red!25}-153 & 	\cellcolor{myGreen!25}324 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}364 & 	\cellcolor{red!25}-784	\\ \thickhline
$\Huge\boldsymbol{H_2}$ & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{red!25}-225 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{myGreen!25}79	\\ \thickhline
$\Huge\boldsymbol{H_3}$ & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{red!25}-225 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{myGreen!25}79	\\ \thickhline
$\Huge\boldsymbol{H_4}$ & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{red!25}-225 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{myGreen!25}79	\\ \thickhline
$\Huge\boldsymbol{H_5}$ & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{red!25}-225 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{myGreen!25}79	\\ \thickhline
$\Huge\boldsymbol{H_6}$ & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{red!25}-225 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{myGreen!25}79	\\ \thickhline
$\Huge\boldsymbol{H_7}$ & 	\cellcolor{red!25}-52 & 	\cellcolor{red!25}-52 & 	\cellcolor{myGreen!25}79 & 	\cellcolor{red!25}-96 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{red!25}-130 & 	\cellcolor{red!25}-208 & 	\cellcolor{red!25}-52 & 	\cellcolor{red!25}-52 & 	\cellcolor{red!25}-46 & 	\cellcolor{red!25}-161 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{red!25}-130 & 	\cellcolor{red!25}-126	\\ \thickhline
$\Huge\boldsymbol{H_8}$ & 	\cellcolor{red!25}-1 & 	\cellcolor{red!25}-1 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}274 & 	\cellcolor{myGreen!25}44 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-63 & 	\cellcolor{red!25}-107 & 	\cellcolor{red!25}-143 & 	\cellcolor{red!25}-143 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}44 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-63 & 	\cellcolor{red!25}-8	\\ \thickhline
$\Huge\boldsymbol{H_9}$ & 	\cellcolor{red!25}-106 & 	\cellcolor{red!25}-106 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{red!25}-36 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-228 & 	\cellcolor{red!25}-280 & 	\cellcolor{red!25}-143 & 	\cellcolor{red!25}-143 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{red!25}-36 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-228 & 	\cellcolor{red!25}-254	\\ \thickhline
$\Huge\boldsymbol{H_{10}}$ & 	\cellcolor{red!25}-13 & 	\cellcolor{red!25}-13 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}34 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-83 & 	\cellcolor{red!25}-128 & 	\cellcolor{red!25}-143 & 	\cellcolor{red!25}-143 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}34 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-83 & 	\cellcolor{red!25}-38	\\ \thickhline
$\Huge\boldsymbol{H_{11}}$ & 	\cellcolor{myGreen!25}12 & 	\cellcolor{myGreen!25}12 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}53 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-44 & 	\cellcolor{red!25}-87 & 	\cellcolor{myGreen!25}12 & 	\cellcolor{myGreen!25}12 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{myGreen!25}53 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{red!25}-44 & 	\cellcolor{myGreen!25}21	\\ \thickhline
$\Huge\boldsymbol{H_{12}}$ & 	\cellcolor{red!25}-1 & 	\cellcolor{red!25}-1 & 	\cellcolor{red!25}-23 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}51 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{red!25}-57 & 	\cellcolor{red!25}-116 & 	\cellcolor{red!25}-1 & 	\cellcolor{red!25}-1 & 	\cellcolor{myGreen!25}142 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}51 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{red!25}-57 & 	\cellcolor{red!25}-8	\\ \thickhline
$\Huge\boldsymbol{H_{13}}$ & 	\cellcolor{red!25}-1 & 	\cellcolor{red!25}-1 & 	\cellcolor{red!25}-23 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}51 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{red!25}-57 & 	\cellcolor{red!25}-116 & 	\cellcolor{red!25}-1 & 	\cellcolor{red!25}-1 & 	\cellcolor{myGreen!25}142 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}51 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{red!25}-57 & 	\cellcolor{red!25}-8	\\ \thickhline
$\Huge\boldsymbol{H_{14}}$ & 	\cellcolor{red!25}-85 & 	\cellcolor{red!25}-85 & 	\cellcolor{red!25}-442 & 	\cellcolor{red!25}-1091 & 	\cellcolor{myGreen!25}122 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-67 & 	\cellcolor{red!25}-410 & 	\cellcolor{red!25}-85 & 	\cellcolor{red!25}-85 & 	\cellcolor{red!25}-100 & 	\cellcolor{red!25}-1091 & 	\cellcolor{myGreen!25}122 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-67 & 	\cellcolor{red!25}-185	\\ \thickhline
$\Huge\boldsymbol{H_{15}}$ & 	\cellcolor{myGreen!25}30 & 	\cellcolor{myGreen!25}30 & 	\cellcolor{red!25}-442 & 	\cellcolor{red!25}-319 & 	\cellcolor{myGreen!25}209 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}111 & 	\cellcolor{red!25}-223 & 	\cellcolor{myGreen!25}30 & 	\cellcolor{myGreen!25}30 & 	\cellcolor{myGreen!25}22 & 	\cellcolor{red!25}-319 & 	\cellcolor{myGreen!25}209 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}111 & 	\cellcolor{myGreen!25}82	\\ \thickhline
$\Huge\boldsymbol{H_{16}}$ & 	\cellcolor{red!25}-23 & 	\cellcolor{red!25}-23 & 	\cellcolor{red!25}-442 & 	\cellcolor{red!25}-412 & 	\cellcolor{myGreen!25}169 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}29 & 	\cellcolor{red!25}-309 & 	\cellcolor{red!25}-23 & 	\cellcolor{red!25}-23 & 	\cellcolor{red!25}-34 & 	\cellcolor{red!25}-412 & 	\cellcolor{myGreen!25}169 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}29 & 	\cellcolor{red!25}-41	\\ \thickhline
$\Huge\boldsymbol{H_{17}}$ & 	\cellcolor{red!25}-29 & 	\cellcolor{red!25}-29 & 	\cellcolor{red!25}-442 & 	\cellcolor{red!25}-422 & 	\cellcolor{myGreen!25}164 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-319 & 	\cellcolor{red!25}-29 & 	\cellcolor{red!25}-29 & 	\cellcolor{red!25}-40 & 	\cellcolor{red!25}-422 & 	\cellcolor{myGreen!25}164 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-55	\\ \thickhline
$\Huge\boldsymbol{H_{18}}$ & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{red!25}-225 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{myGreen!25}79	\\ \thickhline
$\Huge\boldsymbol{H_{19}}$ & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{red!25}-225 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}28 & 	\cellcolor{myGreen!25}20 & 	\cellcolor{red!25}-321 & 	\cellcolor{myGreen!25}208 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}109 & 	\cellcolor{myGreen!25}79	\\ \thickhline
$\Huge\boldsymbol{H_{20}}$ & 	\cellcolor{myGreen!25}8 & 	\cellcolor{myGreen!25}8 & 	\cellcolor{red!25}-107 & 	\cellcolor{red!25}-804 & 	\cellcolor{myGreen!25}285 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}160 & 	\cellcolor{red!25}-367 & 	\cellcolor{myGreen!25}8 & 	\cellcolor{myGreen!25}8 & 	\cellcolor{red!25}-107 & 	\cellcolor{red!25}-804 & 	\cellcolor{myGreen!25}285 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}160 & 	\cellcolor{myGreen!25}44	\\ \thickhline
$\Huge\boldsymbol{H_{21}}$ & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{red!25}-258 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{myGreen!25}200	\\ \thickhline
$\Huge\boldsymbol{H_{22}}$ & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{red!25}-258 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{myGreen!25}200	\\ \thickhline
$\Huge\boldsymbol{H_{23}}$ & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{red!25}-258 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{myGreen!25}200	\\ \thickhline
$\Huge\boldsymbol{H_{24}}$ & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{red!25}-258 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{myGreen!25}75 & 	\cellcolor{red!25}-36 & 	\cellcolor{red!25}-686 & 	\cellcolor{myGreen!25}336 & 	\cellcolor{white}0 & 	\cellcolor{red!25}-723 & 	\cellcolor{red!25}-723 & 	\cellcolor{myGreen!25}265 & 	\cellcolor{myGreen!25}200	\\ 
    \arrayrulecolor{black}\thickhline
\end{tabular}
 }

==> Economic Valuation and Pricing of Inertia in Inverter-Dominated Power Systems - Journal Paper (Matthieu)/tables/table3.tex <==
\huge
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c"c}
    \thickhline
    \cellcolor{black!10}$\Huge\boldsymbol{H\text{\textbackslash}G}$& $\Huge\boldsymbol{G_1}$ & $\Huge\boldsymbol{G_2}$ & $\Huge\boldsymbol{G_3}$ & $\Huge\boldsymbol{G_4}$ & $\Huge\boldsymbol{G_5}$ & $\Huge\boldsymbol{G_6}$ & $\Huge\boldsymbol{G_7}$ & $\Huge\boldsymbol{G_8}$ & $\Huge\boldsymbol{G_9}$ & $\Huge\boldsymbol{G_{10}}$ & $\Huge\boldsymbol{G_{11}}$ & $\Huge\boldsymbol{G_{12}}$ & $\Huge\boldsymbol{G_{13}}$ & $\Huge\boldsymbol{G_{14}}$ & $\Huge\boldsymbol{G_{15}}$ & $\Huge\boldsymbol{G_{16}}$ & $\Huge\boldsymbol{G_{17}}$ & $\Huge\boldsymbol{G_{18}}$ & $\Huge\boldsymbol{G_{19}}$ & $\Huge\boldsymbol{G_{20}}$ \\
    \thickhline
$\Huge\boldsymbol{H_1}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_2}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_3}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_4}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_5}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_6}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_7}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{myGreen!25}3966 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_8}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}274 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_9}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{10}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{11}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}338 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{myGreen!25}4424 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{12}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{13}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{myGreen!25}4195 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{14}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{15}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{16}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{17}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{18}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{19}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{20}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{21}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{22}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{23}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\ \thickhline
$\Huge\boldsymbol{H_{24}}$ & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0 & 	\cellcolor{white}0	\\
    \arrayrulecolor{black}\thickhline
\end{tabular}
 }
